CAE-Bench: Benchmarking AI Agents for Reusable CAE Solver Development

We developed CAE-Bench, a benchmark to evaluate AI agents on Computer-Aided Engineering (CAE) solver development. A CAE solver is more than a PDE solver; it must be able to generalize across various inputs, such as different boundary conditions, geometries, and material properties. CAE-Bench evaluates the generalizability of AI-developed CAE solvers by providing the same task, such as a heat transfer problem, multiple cases, with each case specifying an input. The AI agent develops a solver for a fixed task using only a few public cases, and the resulting solver is then tested on held-out cases, i.e., cases it has never seen before. We evaluate 15 models across a range of reasoning settings on 80 computational tasks. Our experiments show that even if a solver developed by an AI agent performs well on the public cases, it may even get $0$ score on held-out cases. Even GPT-6.2 Astra, the highest-scoring model in our evaluation, averages 42.48 on held-out cases for tasks with varying physical inputs. A data format and an SDK for task registration are provided, so the researcher can use the benchmark on their own infrastructure. We hope that CAE-Bench will help the community to develop AI agents that can develop reusable CAE solvers that generalize to various inputs.

==> tables/cavity_reference_checks.tex <==
\begin{table}[!htbp]
\centering
\small
\begin{tabularx}{\linewidth}{@{}Xrrr@{}}
\toprule
Recorded comparison & \(u\) NRMSE & \(v\) NRMSE & \(p\) NRMSE \\
\midrule
Spatial refinement, L1--L2 & \(1.859\times10^{-3}\) & \(2.596\times10^{-3}\) & \(8.688\times10^{-3}\) \\
Halved time step & \(9.846\times10^{-5}\) & \(1.434\times10^{-4}\) & \(2.024\times10^{-5}\) \\
OpenFOAM, N64 & \(2.226\times10^{-3}\) & \(3.790\times10^{-3}\) & \(7.345\times10^{-3}\) \\
OpenFOAM, N128 & \(2.688\times10^{-3}\) & \(4.267\times10^{-3}\) & \(5.994\times10^{-3}\) \\
\bottomrule
\end{tabularx}
\caption{Recorded consistency checks for each field of the RC7 fixed-cavity reference results (\texttt{cc-lid-driven-cavity}). The hash of the selected reference results matches the historical certificate. These NRMSE values are not newly computed RMS case scores.}
\label{tab:cavity-reference-checks}
\end{table}


==> tables/experiment_cohorts.tex <==
\begin{table}[!htbp]
  \centering
  \small
  \begin{tabularx}{\linewidth}{@{}Xrrrrr@{}}
    \toprule
    Comparison              & \shortstack{Model\\cases} & PDE & \shortstack{Fluid\\mechanics} & Fixed-problem & Cases \\
    \midrule
    Medium model comparison & 6                         & 13  & 32                            & 24            & 554   \\
    Luna effort comparison  & 12                        & 13  & 43                            & 24            & 630   \\
    Score--cost comparison  & 17                        & 13  & 32                            & 24            & 554   \\
    \bottomrule
  \end{tabularx}
  \caption{Tasks included in each comparison. Within each row, every model case is evaluated on the same tasks.}
  \label{tab:experiment-cohorts}
\end{table}


==> tables/full_suite_results.tex <==
\begin{table}[!htbp]
  \centering
  \small
  \begin{tabularx}{\linewidth}{@{}Xlr@{}}
    \toprule
    Model               & Effort & 80-task score \\
    \midrule
    GPT-5.6 Luna        & none   & 34.63         \\
    GPT-5.6 Luna        & low    & 36.81         \\
    GPT-5.6 Luna        & medium & 40.95         \\
    GPT-5.6 Luna        & high   & 53.58         \\
    GPT-5.6 Luna        & xhigh  & 57.77         \\
    GPT-5.6 Luna        & max    & 59.32         \\
    GPT-6 Luna          & none   & 32.52         \\
    GPT-6 Luna          & low    & 40.67         \\
    GPT-6 Luna          & medium & 47.82         \\
    GPT-6 Luna          & high   & 52.58         \\
    GPT-6 Luna          & xhigh  & 56.35         \\
    GPT-6 Luna          & max    & 54.22         \\
    GPT-6 Sol           & medium & 57.93         \\
    GPT-6.1 Sol         & medium & 65.24         \\
    GPT-6.2 Sol & medium & 64.98 \\
    GPT-6.2 Astra & medium & 66.10 \\
    DeepSeek V4.1 Flash & high   & 50.41         \\
    \bottomrule
  \end{tabularx}
  \caption{Scores over all 80 computational tasks. We include model cases with valid reports for every computational task. Infrastructure tests are excluded. These scores cover a different task set from Table~\ref{tab:medium-results}.}
  \label{tab:full-suite-results}
\end{table}

